Image-to-Image Translation with Conditional Adversarial Networks

We investigate conditional adversarial networks as a general-purpose solution to image-to-image translation problems. These networks not only learn the mapping from input image to output image, but also learn a loss function to train this mapping. This makes it possible to apply the same generic approach to problems that traditionally would require very different loss formulations. We demonstrate that this approach is effective at synthesizing photos from label maps, reconstructing objects from edge maps, and colorizing images, among other tasks. Indeed, since the release of the pix2pix software associated with this paper, a large number of internet users (many of them artists) have posted their own experiments with our system, further demonstrating its wide applicability and ease of adoption without the need for parameter tweaking. As a community, we no longer hand-engineer our mapping functions, and this work suggests we can achieve reasonable results without hand-engineering our loss functions either.

==> figs/cityscapes_image_to_labels_latex/fig.tex <==
\begin{figure}

\bgroup 
 \def\arraystretch{0.2} 
 \setlength\tabcolsep{0.2}
\begin{tabular}{cccc}
\begin{center}
Input & Ground truth & L1 & cGAN \\ 
\includegraphics[width=0.25\linewidth]{figs/cityscapes_image_to_labels_latex/input_lindau_000000_000019_leftImg8bit.jpg} &
\includegraphics[width=0.25\linewidth]{figs/cityscapes_image_to_labels_latex/gt_lindau_000000_000019_leftImg8bit.jpg} &
\includegraphics[width=0.25\linewidth]{figs/cityscapes_image_to_labels_latex/L1_lindau_000000_000019_leftImg8bit.jpg} &
\includegraphics[width=0.25\linewidth]{figs/cityscapes_image_to_labels_latex/cGAN_lindau_000000_000019_leftImg8bit.jpg} \\ 
\includegraphics[width=0.25\linewidth]{figs/cityscapes_image_to_labels_latex/input_frankfurt_000001_044525_leftImg8bit.jpg} &
\includegraphics[width=0.25\linewidth]{figs/cityscapes_image_to_labels_latex/gt_frankfurt_000001_044525_leftImg8bit.jpg} &
\includegraphics[width=0.25\linewidth]{figs/cityscapes_image_to_labels_latex/L1_frankfurt_000001_044525_leftImg8bit.jpg} &
\includegraphics[width=0.25\linewidth]{figs/cityscapes_image_to_labels_latex/cGAN_frankfurt_000001_044525_leftImg8bit.jpg} %\\ 
\includegraphics[width=0.25\linewidth]{figs/cityscapes_image_to_labels_latex/input_munster_000113_000019_leftImg8bit.jpg} &
\includegraphics[width=0.25\linewidth]{figs/cityscapes_image_to_labels_latex/gt_munster_000113_000019_leftImg8bit.jpg} &
\includegraphics[width=0.25\linewidth]{figs/cityscapes_image_to_labels_latex/L1_munster_000113_000019_leftImg8bit.jpg} &
\includegraphics[width=0.25\linewidth]{figs/cityscapes_image_to_labels_latex/cGAN_munster_000113_000019_leftImg8bit.jpg} %\\ 
\includegraphics[width=0.25\linewidth]{figs/cityscapes_image_to_labels_latex/input_frankfurt_000000_004617_leftImg8bit.jpg} &
\includegraphics[width=0.25\linewidth]{figs/cityscapes_image_to_labels_latex/gt_frankfurt_000000_004617_leftImg8bit.jpg} &
\includegraphics[width=0.25\linewidth]{figs/cityscapes_image_to_labels_latex/L1_frankfurt_000000_004617_leftImg8bit.jpg} &
\includegraphics[width=0.25\linewidth]{figs/cityscapes_image_to_labels_latex/cGAN_frankfurt_000000_004617_leftImg8bit.jpg}

\end{center}
\end{tabular} \egroup 

\vspace{-0.1in}
\caption{Applying a conditional GAN to semantic segmentation. The cGAN produces sharp images that look at glance like the ground truth, but in fact include many small, hallucinated objects.}
\label{cityscapes_image_to_labels}
\end{figure}

==> figs/facades2_loss_variations_latex/fig.tex <==
\begin{figure*}
\begin{center}$
\bgroup 
 \def\arraystretch{0.2} 
 \setlength\tabcolsep{0.2}
\begin{tabular}{ccccc}
Input & Ground truth & L1 & cGAN & L1 + cGAN \\ 
\includegraphics[width=0.2\linewidth]{figs/facades2_loss_variations_latex/input_46.jpg} &
\includegraphics[width=0.2\linewidth]{figs/facades2_loss_variations_latex/gt_46.jpg} &
\includegraphics[width=0.2\linewidth]{figs/facades2_loss_variations_latex/L1_46.jpg} &
\includegraphics[width=0.2\linewidth]{figs/facades2_loss_variations_latex/cGAN_46.jpg} &
\includegraphics[width=0.2\linewidth]{figs/facades2_loss_variations_latex/L1cGAN_46.jpg} \\ 
\includegraphics[width=0.2\linewidth]{figs/facades2_loss_variations_latex/input_60.jpg} &
\includegraphics[width=0.2\linewidth]{figs/facades2_loss_variations_latex/gt_60.jpg} &
\includegraphics[width=0.2\linewidth]{figs/facades2_loss_variations_latex/L1_60.jpg} &
\includegraphics[width=0.2\linewidth]{figs/facades2_loss_variations_latex/cGAN_60.jpg} &
\includegraphics[width=0.2\linewidth]{figs/facades2_loss_variations_latex/L1cGAN_60.jpg}

\end{tabular} \egroup 
\end{center}
\caption{Loss variations}
\label{facades_loss_variations_qualitative}
\end{figure*}

==> figs/handbags_sketches_lotsofresults_latex/fig.tex <==
\begin{figure*}[width=0.75\linewidth]
\begin{center}
\bgroup 
 \def\arraystretch{0.2} 
 \setlength\tabcolsep{0.2pt}
\begin{tabular}{cccc}
Input & Output & Input & Output \\ 
\includegraphics[width=0.16666666666667\linewidth]{figs/handbags_sketches_lotsofresults_latex/input_13223.jpg} &
\includegraphics[width=0.16666666666667\linewidth]{figs/handbags_sketches_lotsofresults_latex/L1cGAN_13223.jpg} \hspace{0.025in} &
\includegraphics[width=0.16666666666667\linewidth]{figs/handbags_sketches_lotsofresults_latex/input_13252.jpg} &
\includegraphics[width=0.16666666666667\linewidth]{figs/handbags_sketches_lotsofresults_latex/L1cGAN_13252.jpg} \\ 
\includegraphics[width=0.16666666666667\linewidth]{figs/handbags_sketches_lotsofresults_latex/input_13240.jpg} &
\includegraphics[width=0.16666666666667\linewidth]{figs/handbags_sketches_lotsofresults_latex/L1cGAN_13240.jpg} \hspace{0.025in} &
\includegraphics[width=0.16666666666667\linewidth]{figs/handbags_sketches_lotsofresults_latex/input_746.jpg} &
\includegraphics[width=0.16666666666667\linewidth]{figs/handbags_sketches_lotsofresults_latex/L1cGAN_746.jpg} \\ 
\includegraphics[width=0.16666666666667\linewidth]{figs/handbags_sketches_lotsofresults_latex/input_13248.jpg} &
\includegraphics[width=0.16666666666667\linewidth]{figs/handbags_sketches_lotsofresults_latex/L1cGAN_13248.jpg} \hspace{0.025in} &
\includegraphics[width=0.16666666666667\linewidth]{figs/handbags_sketches_lotsofresults_latex/input_13256.jpg} &
\includegraphics[width=0.16666666666667\linewidth]{figs/handbags_sketches_lotsofresults_latex/L1cGAN_13256.jpg} \\ 
\includegraphics[width=0.16666666666667\linewidth]{figs/handbags_sketches_lotsofresults_latex/input_798.jpg} &
\includegraphics[width=0.16666666666667\linewidth]{figs/handbags_sketches_lotsofresults_latex/L1cGAN_798.jpg} \hspace{0.025in} &
\includegraphics[width=0.16666666666667\linewidth]{figs/handbags_sketches_lotsofresults_latex/input_13258.jpg} &
\includegraphics[width=0.16666666666667\linewidth]{figs/handbags_sketches_lotsofresults_latex/L1cGAN_13258.jpg}

\end{tabular} \egroup 
\end{center}
\caption{Example results of the edges$\rightarrow$handbags model applied to human-drawn sketches. Note that the model was trained on automatically detected edges, but generalizes to human drawings.}
\label{handbags_sketches_lotsofresults}
\end{figure*}

==> figs/shoes_sketches_lotsofresults_latex/fig.tex <==
\begin{figure*}[width=0.75\linewidth]
\begin{center}
\bgroup 
 \def\arraystretch{0.2} 
 \setlength\tabcolsep{0.2pt}
\begin{tabular}{cccc}
Input & Output & Input & Output \\ 
\includegraphics[width=0.16666666666667\linewidth]{figs/shoes_sketches_lotsofresults_latex/input_14974.jpg} &
\includegraphics[width=0.16666666666667\linewidth]{figs/shoes_sketches_lotsofresults_latex/L1cGAN_14974.jpg} \hspace{0.025in} &
\includegraphics[width=0.16666666666667\linewidth]{figs/shoes_sketches_lotsofresults_latex/input_14985.jpg} &
\includegraphics[width=0.16666666666667\linewidth]{figs/shoes_sketches_lotsofresults_latex/L1cGAN_14985.jpg} \\ 
\includegraphics[width=0.16666666666667\linewidth]{figs/shoes_sketches_lotsofresults_latex/input_15035.jpg} &
\includegraphics[width=0.16666666666667\linewidth]{figs/shoes_sketches_lotsofresults_latex/L1cGAN_15035.jpg} \hspace{0.025in} &
\includegraphics[width=0.16666666666667\linewidth]{figs/shoes_sketches_lotsofresults_latex/input_14971.jpg} &
\includegraphics[width=0.16666666666667\linewidth]{figs/shoes_sketches_lotsofresults_latex/L1cGAN_14971.jpg} \\ 
\includegraphics[width=0.16666666666667\linewidth]{figs/shoes_sketches_lotsofresults_latex/input_14983.jpg} &
\includegraphics[width=0.16666666666667\linewidth]{figs/shoes_sketches_lotsofresults_latex/L1cGAN_14983.jpg} \hspace{0.025in} &
\includegraphics[width=0.16666666666667\linewidth]{figs/shoes_sketches_lotsofresults_latex/input_14980.jpg} &
\includegraphics[width=0.16666666666667\linewidth]{figs/shoes_sketches_lotsofresults_latex/L1cGAN_14980.jpg} \\ 
\includegraphics[width=0.16666666666667\linewidth]{figs/shoes_sketches_lotsofresults_latex/input_15023.jpg} &
\includegraphics[width=0.16666666666667\linewidth]{figs/shoes_sketches_lotsofresults_latex/L1cGAN_15023.jpg} \hspace{0.025in} &
\includegraphics[width=0.16666666666667\linewidth]{figs/shoes_sketches_lotsofresults_latex/input_15011.jpg} &
\includegraphics[width=0.16666666666667\linewidth]{figs/shoes_sketches_lotsofresults_latex/L1cGAN_15011.jpg}

\end{tabular} \egroup 
\end{center}
\caption{Example results of the edges$\rightarrow$shoes model applied to human-drawn sketches. Note that the model was trained on automatically detected edges, but generalizes to human drawings}
\label{shoes_sketches_lotsofresults}
\end{figure*}
